Auto-Icon+: An Automated End-to-End Code Generation Tool for Icon Designs in UI Development

Approximately 50% of development resources are devoted to UI development tasks [9]. Occupying a large proportion of development resources, developing icons can be a time-consuming task, because developers need to consider not only effective implementation methods but also easy-to-understand descriptions. In this paper, we present Auto-Icon+, an approach for automatically generating readable and efficient code for icons from design artifacts. According to our interviews to understand the gap between designers (icons are assembled from multiple components) and developers (icons as single images), we apply a heuristic clustering algorithm to compose the components into an icon image. We then propose an approach based on a deep learning model and computer vision methods to convert the composed icon image to fonts with descriptive labels, thereby reducing the laborious manual effort for developers and facilitating UI development. We quantitatively evaluate the quality of our method in the real world UI development environment and demonstrate that our method offers developers accurate, efficient, readable, and usable code for icon designs, in terms of saving 65.2% implementing time.

==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/acknowledgments.tex <==
\begin{acks}
We appreciate Yanfang Chang, Zixiao Zhao, and Jiawen Huang for designing and conducting a survey experiment, and all the participants from Imgcook team in Alibaba Group for taking surveys.
\end{acks}

==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/approach.tex <==
\begin{figure*}  
	\centering 
	\includegraphics[width=\linewidth]{figs/approachv4.png}  
	\caption{The approach of our tool, \tool. Given a design artifact as input, we first compose the components into icons by clustering, for example, the "eye", "mouth", "face" components are composed into a smiling face icon. We then apply three major functions, involving font conversion, prediction and color detection, to generate the output code for the icon, which consists of a font file (.ttf) and a descriptive tag, for example "icon-emoji" and "blue".}
	\label{fig:approach}
\end{figure*}

\section{Approach}
% According to our findings in Section~\ref{pre_study}, we present \textit{Auto-Icon} to lower the transition barrier (RQ1: icons are assembled from multiple components in design artifact), expedite rendering of icons (RQ2), and increase readability of the icon tags (RQ3), which help facilitating icon implementation process.

Based on the interview study in Section~\ref{pre_study}, we summarized three design considerations for our approach: 
(1) icons are assembled from multiple components in the design artifact.
(2) icons implemented as fonts can expedite rendering.
(3) adding descriptions to icons can increase readability and accessibility of code.



To solve (1), we proposed a machine learning technique to cluster the scattered components in the design artifact through heuristic correlation coefficient and then composed the clusters of components into icons (Section~\ref{iconcomposition}).
To solve (2), we proposed an automated conversion technique, taking an icon as the input, and outputting a vector graphics font(Section~\ref{convertion}). 
% The technique combines computer vision for detecting polygons in the image, and graph algorithm for optimizing curves in the polygons .
To address (3), we got inspired from the findings in our study on icon characteristic in Section~\ref{characteristics} to develop a deep learning model to automatically assign the classes of icons in order to reduce the effort of manually designing the description of icons (Section~\ref{prediction}).
Additionally, we applied a primary color detection method based on computer vision to keep track of the primary color of the icon in order to support more detailed description in code (Section~\ref{detection}). 
The overview of our approach is shown in Fig.~\ref{fig:approach}.




% \begin{table}[ht]
% \caption{A table arranging  images}
% \centering
% \begin{tabular}{p{0.12\linewidth}p{0.45\linewidth}p{0.3\linewidth}p{0.1\linewidth}}
%     \toprule
%     \bf{CLASS} & \bf{ASSOCIATED} & \bf{EXAMPLES} & \bf{NO} \\
%     \midrule
%     \bf{\small flag} & \small{banner, notification} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/4.png}} & 356 \\
%     \bf{\small delete} & \small{remove, trash, clear} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/33.png}} & 525 \\
%     \bf{\small upload} & \small{file-upload, cloud, uploading} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/8.png}} & 432 \\
%     \bf{\small close} & \small{reject, cross, clear, cancel} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/45.png}} & 349 \\
%     \bf{\small time} & \small{alarm, clock, watch, timer, countdown} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/48.png}} & 551 \\
%     \bf{\small data} & \small{database, chart, pie, bar, cloud} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/29.png}} & 398 \\
%     \bf{\small lock} & \small{knit, secure, unlock, password} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/7.png}} & 416 \\
%     \bf{\small weather} & \small{forecast, temperature, conditions} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/51.png}} & 317 \\
%     \bf{\small barcode} & \small{qr-code, scan} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/47.png}} & 419 \\
%     \bf{\small vip} & \small{member, crown} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/2.png}} & 341 \\
%     \bf{\small bluetooth} & \small{connect, wireless} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/22.png}} & 311 \\
%     \bf{\small contact} & \small{group, friends, requests} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/57.png}} & 424 \\
%     \bf{\small wechat} & \small{chat, share, login} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/13.png}} & 419 \\
%     \bf{\small link} & \small{connect, hyperlink} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/6.png}} & 432 \\
    % \bf{\small key} & \small{password, open, authority} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/38.png}} & 378 \\
    % \bf{\small scan} & \small{radar, qrscan, ocr} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/14.png}} & 421 \\
%     \bottomrule
% \end{tabular}
% \label{tab:gt}
% \end{table}











\subsection{Icon Composition}
\label{iconcomposition}

\begin{algorithm}[t]
    \linespread{0.2}
	\SetAlgoLined
	\SetNoFillComment
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{UI design artifact $X$ with $n$ elements $\{x_1, x_2, x_3, ..., x_n\}$}
	\Output{Hierarchical Dendrogram $HD$}
	construct $n \times n$ matrix $HD$ with correlation metric $cor(i,j)$ between the elements \;
	\While{len($X$) > 1}{
	    Select the pair $(x_i,x_j)$ with the largest correlation value, such as $x_i,x_j \in X$ \;
	    Merge the pair $(x_i,x_j)$ into a new cluster $x_{merge}=x_i \cup x_j$, let $x_i,x_j$ be the sub clusters of cluster $x_{merge}$. \;
	    Update $X \gets X \cup \{x_{merge}\} - \{x_i,x_j\}$ \;
	    \ForEach{$x \in X$}{
	        Update the matrix $HD$ with correlation metric $cor(x,x_{merge})$ \;
	    }
	}
	return $HD$
	\caption{Hierarchical Agglomerative Clustering (HAC)}
	\label{algorithm:hac}
\end{algorithm}




% Chung Horng et al9
% . discussed about the HAC
% Hierarchical Agglomerative Clustering for the wireless
% sensor network. HAC is a conceptually and mathematically simple clustering approach. HAC has two important
% categories, divisive and agglomerative.

% Hierarchical routing is the procedure of arranging nodes
% in a hierarchical manner. It is one of the most popular
% researches in WSNs, and many typical algorithms are proposed.

% The motivation of our research is to provide efficient
% clustering without requiring the global knowledge of network by reversing the clustering approach from top-down
% to bottom-up. With the bottom-up approach, sensor nodes
% collaborate and build clusters before they select CHs. In
% this manner, the bottom-up approach can be a better
% way to implement self-organization, scalability and flexibility. 





% Normally, the assumed number of clusters may be
% unreliable since the nature of the grouping structures among the data is unknown
% before processing and thus the partitioning methods would not predict the structures of the data very well. Hierarchical clustering has been chosen to solve this problem by which they provide data-views at different levels of abstraction, making them ideal for people to visualize the concepts generated and interactively explore large document collections. 

% Unlike partitional clustering algorithms that build a hierarchical solution from top to
% bottom, repeatedly splitting existing clusters, agglomerative algorithms build the
% solution by initially assigning each document to its own cluster and then repeatedly selecting and merging pairs of clusters, to obtain a single all-inclusive cluster,
% generating the cluster tree from leaves to root [11]. 


The most common way to group related pieces is through clustering.
Normally, the assumed number of clusters may be unreliable since the number of the icons among the design artifact is unknown and thus the top-down partitioning methods (i.e., K-Means~\cite{likas2003global}, Expectation-Maximization~\cite{dempster1977maximum}, etc.) will not applicable.
To provide clustering without requiring the knowledge of clusters, we adopted a bottom-up approach Hierarchical Agglomerative Clustering (HAC)~\cite{murtagh2014ward}.
The details of HAC is shown in Algorithm~\ref{algorithm:hac}, where each component in the design artifact is treated as a singleton cluster to start with and then they are successively merged into pairs of clusters until all components have merged into one single large cluster.
The main parameters in this algorithms are the metric used to compute the correlation value of components, which determines the pair of clusters to be merged at each step.
According to our observations in Section~\ref{em_rq1}, we defined a heuristic correlation metric that takes into account component's attribute, hierarchy, and rendering:
\begin{equation}
	Correlation(x,y) = \alpha \times ATTR(x,y) + \beta \times HRCHY(x,y) + \gamma \times IOU(x,y)
	\label{eq:correlation}
\end{equation}
where $ATTR(x,y)$ measures the attribute type of two components $x,y$, that is if they have same type (i.e., image, curve, shape, etc.), it assigns the value to 1 else 0.
$HRCHY(x,y)$ measures the hierarchy between components, the value is assigned to 1 if they are under the same group, 0 otherwise.
$IOU(x,y)$ measures the overlap between components, taking a value between 0 to 1.
And $\alpha, \beta, \gamma$ is the user-defined weights for each measurements.
The higher the correlation value, the more likely the cluster can composed to an icon.
% We empirically choose 0.5 as the $w$ value for the best performance. 


\begin{figure*}  
	\centering 
	\includegraphics[width=0.75\linewidth]{figs/hac.png}  
	\caption{The HAC clustering algorithm to compose components into icons in the design artifacts, that repeatedly selecting and merging pairs of clusters based on a heuristic correlation metric, until a single all-inclusive cluster (UI). By empirically setting a correlation threshold to 0.6 and distinguishing icon cluster by its feature as discussed in Section~\ref{empiricalstudy} (small, transparent and low contrast), the blue cluster is determined as an icon.}
	\label{fig:hac-example}
\end{figure*}

The agglomeration of clusters results in a tree-like structure called the dendrogram as shown in Fig~\ref{fig:hac-example}.
The value is highest at the lowest level of the dendrogram and it decreases as the clusters merge into the final single cluster. 
By cutting the dendrogram at an empirically setting of value threshold (e.g., 0.6), we may retrieved several clusters, for example, the icon (blue cluster), text (red cluster), and background (green cluster) in Fig~\ref{fig:hac-example}.
To further identify if the aggregated cluster is an icon (blue cluster), we followed the feature of icon discussed in Section~\ref{empiricalstudy}, that the icon should be small and low contrast.

% This
% structure can then be used to extract partitions of the data set
% by cutting the dendrogram at the required level of
% combination similarity or number of clusters expected. Fig. 2
% shows such a dendrogram illustrating the HAC algorithm,
% where the singleton clusters p, q, r, s a














\subsection{Font Conversion from Icon}
\label{convertion}
% The process of converting from font to image is simple. The converse process which takes an image to font is not simple, also known as image tracing problem to trace an approximation of the original image.
Unlike converting font to image, transcribing image to font, which is also known as image tracing problem, is a difficult task.
% Recently, the performance of tracing algorithm is further boosted by exploiting the techniques uniting computer vision and computer graphics~\cite{orzan2008diffusion,yao2014improved,fayaza2016resolution,dominici2020polyfit}.
% There are a variety of algorithms to perform results by concerning uniting computer graphics and computer vision techniques~\cite{??}.
In this work, we adopted the state-of-the-art Potrace~\cite{selinger2003potrace} in Fig~\ref{fig:approach}A.
% Figure~\ref{fig:approach}A presents the overall process of the algorithm.
% , involving three steps: edge detection, polygon optimization, and smoothing
We first applied a pre-processing method for converting color to binary (i.e., black and white) image by setting a threshold to control the bit of each pixel after calculating the average value in three channels \((R + G + B) / 3 \).
We regarded the pixel is of white if the average value is larger than 128, while black if the value is equal to or smaller than 128.
Then, we detected the edge in the black-white image.
An edge is defined to be a border between a white pixel and a black pixel, which indicate which pixels from the original image constitute the borders of region.
Note that the edge is assigned a direction so that when moving from the first endpoint to the second, the black pixel is on the left (as shown in Fig~\ref{fig:approach}A edge detection).
This process was repeated until we reached the starting point, at which point we have found a closed path which encloses a black region.
Once the border was found, we approximated/optimized the border with a polygon to figure out which border pixels is possible to connect with a straight line such that the line passes through all the border pixels between its endpoints. 
To detect the optimal polygon, we computed a penalty value to measure the average distance from the edge to the pixels it approximates. 
The polygon with the smallest penalty (equivalent to the polygon with the fewest pixels) is the optimal one.
Finally, we used a cubic curve defined by four control points (also known as Bezier curve~\cite{sederberg1992approximation}) to smooth the corners.
The first and fourth control points (i.e., midpoints of the edges of the polygon) give the locations of the two endpoints of the curve, while the second and third (i.e., chosen on the polygon edges through the endpoints) indicate the direction and magnitude of the derivative of the curve at each endpoint.


\subsection{Prediction for Icon}
\label{prediction}
Traditional Convolutional Nerual Network (CNN)~\cite{lecun1998gradient, krizhevsky2012imagenet} has shown great potential as a solution for difficult vision problems.
MobileNetV2~\cite{sandler2018mobilenetv2} distills the best practices in convolutional network design into a simple architecture that can serve as competitive performance but keep low parameters and mathematical operations to reduce computational power.
The architecture of the network is shown in Fig~\ref{fig:approach}B.

Instead of using regular convolutional layers widely used in traditional CNN architectures to capture essential information from images but are expensive to compute, MobileNetV2 adopted a more advanced one, depthwise separable convolutions.
Depthwise separable convolution combined a $3*3$ convolution layer and two $1*1$ convolution layers.
The $1*1$ convolution layer (also named as pointwise convolution layer) was used to combine the filter values into new features, while the $3*3$ convolution (also called as depthwise convolution layer) was used to filter the input feature map.
Inspired from the dimension augmentation in the work of~\cite{lin2013network}, MobileNetV2 used a $1*1$ pointwise convolution layer to expand the number of channels in the input feature map.
Then it used a $3*3$ depthwise convolution layer to filter the input feature map and a $1*1$ convolution layer to reduce the number of channels of feature map.
The network borrowed the idea of residual connection in ResNet~\cite{he2016deep} to help with the flow of gradients.
In addition, batch normalization and activation layer were added between each depthwise convolution layer and pointwise convolution layer to make the network more stable during training.
For detailed implementation, we adopted the stride of 2 in the depthwise convolution layer to downsample the feature map.
For the first two activation layers, the network used ReLU6 defined as $y=min(max(0,x),6)$ because of its robustness in low-precision computation~\cite{howard2017mobilenets}, and a linear transformation (also known as Linear Bottleneck Layer) was applied to the last activation layer to prevent ReLU from destroying features.
% To make our training more stable, we used a constant learning schedule with rate 0.001, adopted Adam as an optimizer~\cite{kingma2014adam}, and CrossEntropyLoss as the loss function~\cite{murphy2012machine}.
% For each image, we normalized the pixel value by dividing the mean and standard deviation so that each pixel value is in the range between 0 to 1 for accelerating the training process.


\subsection{Color Detection of Icon}
\label{detection}
Since the conversion between icon and font sacrifices the color identity, we added an attribute to keep track of the primary color of the icon.
% An usage feature that developers suggest in our study is to annotate icon image with color label, because color is an important aspect of description.
To that end, we adopted HSV colorspace for color detection.
We first removed the fourth alpha channel as transparent and made a conversion from RGB color to HSV colorspace. Each RGB color has a range of HSV vale. The lower range is the minimum shade of the color that will be detected, and the upper range is the maximum shade. 
For example, blue is in the range of $\langle 100,43,46 \rangle$--$\langle 124,255,255 \rangle$.
Then, we created a mask for each color (black, blue, cyan, green, lime, megenta, red, white) as shown in Fig.~\ref{fig:approach}C. 
The mask is the areas that HSV value on pixels match the color between the lower range and upper range. 
Finally, we calculated the area of the mask in each color and the corresponding image occupancy ratio. 
The color with the maximum ratio was identified as the primary color of the icon (the blue in the example in Fig.~\ref{fig:approach}C).



\begin{comment}
\subsection{MoibleNet V2}
\begin{figure}[h]
\includegraphics[width=8cm]{figs/V1_block.png}
\label{v1_block}
\caption{The architecture of Depthwise Separable Convolution Block in MobileNet V1}
\end{figure}

Introduced by Google, MobileNet is a neural network architecture that aims to reduce computational power.
Compare with traditional CNN architecture, MobileNet shows similar\sidong{competitive} performance while keeping low parameters and mathematical operations.
Regular convolutional layers, which are widely used in traditional CNN architectures,  are important to capture essential information from images but are expensive to compute.
By depthwise separable convolutions, MobileNet V1 highly reduce the computational requirement but still keep the ability of capturing essential information.
Unlike traditional convolution, depthwise separable convolution includes $3*3$  convolution layer and $1*1$ convolution layer.
The $3*3$ convolution, which is called depthwise convolution layer, is used to filter the input feature map, and the $1*1$ convolution layer, which is  called pointwise convolution layer, is used to combine the filter values into new features.
Fig \ref{v1_block} shows the structure of MobileNet V1 depthwise separable convolution block .
Bath Normalization and RuLU6 activation layer are added between each depthwise convolution layer and pointwise convolution layer.
The RuLU6 is defined as follow:
$$y=min(max(0,x),6)$$
Compared with regular convolution layers, the depthwise and pointwise convolution layer possess the same functionality but use less computational resources.
In MobileNet V1, pooling layer are not used between these depthwise separable blocks.
To reduce the spatial dimensions of the input feature map, some depthwise convolution layer have stride of 2.\\

\begin{figure}[h]
\includegraphics[width=8cm]{figs/V2_block.png}
\label{v2_block}
\caption{The architecture of Depthwise Separable Convolution Block in MobileNet V2}
\end{figure}

To improve the efficiency of MobileNet V1, MobileNet V2 is designed with more advanced structures.
As shown in Fig \ref{v2_block}, the depthwise separable convolution block is redesigned.
Compared with MobileNet V1, three new layers are introduced in the new convolution block.
Firstly, in order to expand the number of channels in the input feature map, $1*1$ convolution layer is used before the the depthwise convolution layer.
Secondly, a $3*3$ depthwise convolution layer is used to filter the input feature map.
Thirdly, another $1*1$ convolution layer is used to reduce the number of channels of feature map.
Since the last layer reduce the number of data that flow to next layer, it is also called bottleneck layer.\\



\begin{table}
\centering
    \begin{tabular}{|c|c|c|} 
    \hline 
    Layer&Type&Ouput Size\\
    \hline  
    0& $3 \times 3$ regular convolution layer& $112 \times 112 \times 32$\\
    \hline 
    1& depthwise separable convolution block& $112 \times 112 \times 16$\\
    \hline 
    2-3& depthwise separable convolution block& $56 \times 56 \times 24$\\
    \hline 
    4-6& depthwise separable convolution block& $28 \times28 \times 32$\\
    \hline 
    7-10& depthwise separable convolution block& $14 \times14 \times 64$\\
    \hline 
    7-10& depthwise separable convolution block& $14 \times14 \times 96$\\
    \hline 
    14-16& depthwise separable convolution block& $7 \times7 \times 160$\\
    \hline 
    17& depthwise separable convolution block& $7 \times7 \times 320$\\
    \hline 
    18& $1 \times 1$ regular convolution layer & $7 \times 7 \times 1280$\\
    \hline 
    \end{tabular}
\caption{Full architecture of MobileNet V2}
\label{tab:v2_s}
\end{table}

To fully use the information of feature map and help with the flow of gradients, residual connection is used in MobileNet V2 as ResNet \suyu{ref}.
In the first two layers, batch normalization and ReLU6 are used as activation function.
In the last layer, only batch normalization is used since non-linear function lead to miss of information.
The full architecture of MobileNet V2 is shown in table \ref{tab:v2_s}.
The first layer is a $3*3$ regular convolution layer. 
Then 17 new depthwise separable blocks are used.
The last layer is a $1*1$ regular convolution layer.\\
\end{comment}









==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/conclusion.tex <==
\section{Conclusion}
% In this paper, we present a deep-learning and computer vision approach that can provide developers with intelligent support to reduce the development time of icon design in the UI.
% The core techniques are three-fold.
% First, we develop an automated image convertion method to turn an icon image into a font in which improving UI rendering speed. 
% Second, to assist developers with better code accessibility, we adopt a deep learning model to automatically predict the descriptive label that convey the semantics of the icon image.
% Third, according the colorspace of the image, we detect the primary color of the icon to provide developers more knowledge on the image.
% Our method is incorporated into existing automated code generation platform to extend them beyond effective and descriptive coding.


In this paper, we present a novel approach, \tool, that can provide developers with intelligent support to reduce the development time of icon design in the UI.
Our approach consists of two integral parts: a heuristic machine learning methods for icon composition, and a deep learning and computer vision method for icon implementation.
Our work possesses several distinctive advantages:
1) to bridge the conceptual gap between designers and developers in icon, we propose a heuristic-based clustering method to compose the scattered icon pieces in the design artifact into an icon.
2) we develop an automated image conversion method to turn an icon into a font in which improving icon rendering speed. 
3) to assist developers with better code accessibility, we adopt a deep learning model to automatically predict the descriptive label that convey the semantics of the icon.
4) base on the colorspace of the image, we detect the primary color of the icon to provide developers more knowledge on the icon.
Our method is incorporated into existing automated code generation platform to extend them beyond effective and descriptive coding.


==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/discussion.tex <==
\section{Discussion}
% We discuss some implications of our work on developers and generalization of our method.

\textbf{On developers:}

Due to the conceptual gap between designers and developers, there is a transition barrier from design artifact to implementation. Developers require extra effort to compose design components into icons for optimizing the network traffic and caching.
To bridge this transition gap, our work proposes a heuristic machine learning technique to cluster components in the design artifacts to automated agglomerate the scattered icon components into clusters, helping to ease the burden of manual search for developers. The clusters can be further applied to various downstream tasks such as icon implementation, UI testing~\cite{moran2018machine}, css clipping~\cite{larsen2018mastering}, etc.
Icon implementation is a challenging and time-consuming task, even for professional developers.
On the one hand, UI developers must enhance performance.
Poor development has an adverse effect on the performance of the site. 
The performance issues comprise a multitude of factors like rendering speed, reusability \& flow of the code, etc.
On the other hand, UI developers must write a clean, high quality code which can be easily understood and maintained.
Inspired by the high performance of font rendering, our work designs an automated method to convert icon to font using computer vision techniques to trace the edge of icon and using graphic algorithm to optimize the edge.
In addition, compared with the missing descriptions in the development or brainstorming suitable names which is limited to several developers in the physical world, our deep learning and computer vision techniques based method can quickly identify the label and the color of icon.
% In addition, compared with the missing descriptions in the development or brainstorming suitable names which is limited to several developers in the physical world, our method based on deep learning and computer vision techniques can quickly identify the label and the color of icon design.
Our method once made accessible to developers, can very well help developers achieve efficient icon coding.

% \begin{figure}  
% 	\centering 
% 	\includegraphics[width=0.7\linewidth]{figs/interesting.png}  
% 	\caption{Examples of the five novel icon designs.} 
% 	\label{fig:interesting}
% \end{figure}

\textbf{On the generalization of our method:}
We report and analyze the performance of our CNN-based model for predicting icon labels in Section~\ref{prediction_result}. 
One limitation with our model is that we currently only test our model on 100 labels with enough corresponding icons.
With the cooperation with \textit{Imgcook} platform, the icons in the UI images are a gold resource.
First, the icons are relatively unique, otherwise, developers can reuse the online resources directly. These unique icons can significantly increase the amount of data, consequently improving the accuracy of our model.
Second, developers may modify the description to a serendipitous label which can augment the labels and generalize a broader range of icon descriptions.
Due to the time limit, we only collect a small amount of icons from \textit{Imgcook}.
However, we have seen some interesting icons that do not exists on online sharing platforms and they may improve the generalization of our method.

\textbf{Area of improvements:}
% Developers point out various areas in which our method can be improved with.
Currently, we only predict the label based on icon itself. As discussed in Section~\ref{user_study_result}, the meaning of icon varies in different context.
To address this problem, we can consider the entire UI, capturing all the related information to make the final prediction.
Developers praise the idea of adding descriptions to the code which is a tedious task for them.
They wonder whether our model can extend to other elements.
% For example, captioning of image could benefit them from writing descriptions for blind people to support accessibility.
% An developer hope us to support description for buttons who finds that some buttons do not have descriptive texts to explain its intention, resulting in a bad user experience.
An developer hope us to support description for buttons as he finds many buttons do not have descriptive texts to explain its intention, resulting in a bad user experience.
% In order to solve the problem, he needs to manually add a hover text for those buttons.
We believe our model could help developers in this case as it will not be difficult to extend to other elements once we obtain enough data for the training.
Moreover, developers envision the high potential in being able to add icon size descriptions as one of the biggest strength of font is lossless scalability. To that end, we can measure the height of the icon and map it to the corresponding font size.












% \begin{table}[ht] 
% \caption{Stimuli Category Explanations} 
% \label{tab:stimuli}
%   \begin{tabular}{p{0.1\linewidth}p{0.4\linewidth}p{0.4\linewidth}p{0.1\linewidth}} 
%       \hline
%       \bf{CLASS} & \bf{ASSOCIATED} & \bf{EXAMPLES} & \bf{NO}\\
%       \hline 
%       \bf{\small delete} & \small{remove, trash, clear} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/33.png}} & 35 \\
%       \hline
%   \end{tabular}
% %   \tabfnt{Note: Bold categories are biologically correct growth models.}
% \end{table}

==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/empiricalstudy.tex <==
\section{Preliminary Study}
\label{pre_study}
% \textit{1) do developers implement icon images in font or image?} \textit{2) do developers write descriptions for icon image?}
To better understand the challenges in the real-world UI development environment, we conducted an interview with 12 front-end developers from the big companies.
Two authors first developed the interview protocol, and conducted pilot studies with two participants. 
Based on the pilot studies, we refined the interview protocol and conducted 10 interviews formally.
% Their demographic data and their familiarity with UI development can be found in Table~\ref{?}.
The average length of these interviews is 20 minutes.
We started with general questions, such as questions about working years, workload of development, and number of projects developed.
% We then asked the interviewees about the code they implemented for icon images.
Then, we asked the interviewees how they developed the code for icon images.
We particularly asked what motivated them to adopt the approach, whether they revised the implementation, what approaches could achieve the same effect, what they perceived as the impact of the implementation, how the implementation behaved in the process of development and is there any difference on UI development between personal projects and company tasks.
% We particular asked the following questions: 1) What motivates you to adopt the current approach for rendering icons? 2) Do you revise the implementation? 3) Can other approachs achieve the same effect? 4) Why you did not choose the other approach?  5) How good does this approach performance in development process.


\begin{figure*}  
	\centering 
	\includegraphics[width=0.65\linewidth]{figs/icon-example.png}  
	\caption{An illustration of icon design in the design artifact given by designers. A "gift" icon is composed by multiple components such as bitmap, lines, and shapes (highlighted).}
	\label{fig:iconexample}
\end{figure*}

% what icon looks like
\subsection{Research Question 1: do developers implement icons directly from the design artifacts?}
\label{em_rq1}


Once the design artifacts are completed by designers, they are handed off to development teams who are responsible for implementing the designs in code. 
Fig.~\ref{fig:iconexample} shows an example of the design artifact handed off to developers.
The design artifacts are stored as archives containing JSON encoded layout and a number of binary assets such as bitmap images, curves, shapes~\cite{sketch_developer}.
The layout is structured as a cumulative hierarchy comprising a tree structure, starting with a single root node, where the spatial layout of parent always encompasses contained child components.
A discrete component with a corresponding set of attributes can be represented as a five-tuple in the form ($<name>, <x-position,y-position>, <width,height>, <text>, <image>$). 
Here the first element of the tuple describes the name of the component.
The next four elements of the tuple describe the location of the top left point for the bounding box of the component, and the height and width attributes describe the size of the bounding box.
The text attribute corresponds to text displayed (if any) by the component and the image attribute represents an image (if any) of the component with bounds adhering to the position attributes.
% For example, the first highlighted component can be represented as $(<bitmap cover>, <10.0, 213.0>, <40, 20>, <None>, <Image>)$.



All of the developers demonstrated that they always preprocess the icon designs before implementing, due to the gap to designers.
As D9 said that \textit{"We are all fulfilling of our goals, but in different directions."}
At the core of it, designers are focused on the graphical/visual representations of icons, while the developers take care of the functionality of icons, such as efficient rendering.
However, this gap points to a more prominent problem for icon implementation in practice as D10 showcased an icon design in the design artifact (as shown in Fig~\ref{fig:iconexample}) and said:



\textit{
In most big IT or software companies, the visual designers design the UI with professional tools like Sketch~\cite{sketch} or Adobe Photoshop~\cite{ps}.
These tools provide build-in curvature pen/pencil tool allow designers to create some complicated components by drawing smooth curves and straight line segments with equal ease in order to sketch out the desired shape.
Well-designed icons are usually composed of images, curves, lines, shapes, etc.
For example, in Fig~\ref{fig:iconexample}, the "gift" icon is composed by lines, shapes, and bitmaps.
Developers need to spend extra effort to compose all the small pieces into an icon to gain icon rendering efficiency and code accessibility. 
}




% Although designers may organize the resources of an icon with some layout hierarchies to group them (for example "group6" in Fig~\ref{fig:iconexample}), d









They also mentioned that finding all the components of an icon is surprisingly non-trivial task.
This is because that as designers only concern with the visual representation of icon, they may create one icon with many components scattered all over the design artifact. 
For example, the bitmap ("knot-bow") is a component of the "gift" icon but not in the same hierarchy of other components in Fig~\ref{fig:iconexample}.
D9 supported this claim that:




\textit{
Although there is much information (i.e., name, attribute, hierarchical relationship, etc.) in the design artifact, that information does not align well with that required in the icon composition and implementation.
In practice, I potentially consider three characteristics to compose an icon.
First, the rendering of the components of icon should be close/overlap to each other.
Second, some designers may organize the resources of an icon with some layout hierarchies to group them, for example "group6" in Fig~\ref{fig:iconexample}.
Third, some designers may use the same format to name icon components, for example "gift-piece-x".
Therefore, it takes time to search all the components with reference to their rendering, hierarchy, and attribute.
}



\noindent\fbox{
    \parbox{0.98\textwidth}{
        Due to the gap between designers and developers, developers can hardly implement icons from design artifacts directly.
        Given a design artifact, developers require to manually compose the icon image by searching all the related components based on their attributes, hierarchies and renderings, adding to the complexity and effort required to icon implementation in practice.
        % The process is expensive and cumbersome.
    }
}













% in fonts or images?
\subsection{Research Question 2: do developers implement icons in font or images?}
% \begin{itemize}
%     \item <img>
%     \item <a>
%     \item css background img
%     \item font? svg?
% \end{itemize}
By summarising the approaches, we collected 4 ways of rendering icons, i.e., image tag <img> or <svg>, icon tag <i>, css background image, and custom tag <SvgIcon> as shown in Table~\ref{tab:icon_development}.
One third of our developers listed all approaches, 80\% developers knew the way of using image and font.
There are 2 developers who have never heard of or used the fonts to render icons, D2 said:

\textit{Making front-end development is fun, although sometimes it hurts because I do not have adequate learning experience.
There are few front-end courses in universities, and these courses usually contain relatively simple knowledge, such as what is <div> block, how to connect HTML and CSS together, etc.
They do not teach the usage of font, especially they do not distinguish the difference between fonts and images in rendering icons.}

70\% developers implemented icons as image when developing front-end codes based on UI design draft files because they found that converting icon to font is a complicated and laborious process. For example, D7 mentioned:

\textit{To implement the approach of icon font, I first need to upload the image to the existing conversion websites such as icomoon~\cite{icomoon} and Fontello~\cite{fontello}.
Then, I need to download the generated icon font to my local device.
Last but not least, I need to copy the generated CSS code to CSS files.
This entire process requires a lot of time and effort, but due to time constraints, the process is not compatible in industry.}

One developer D2 from Alibaba described how limit the time in their UI development:

\textit{
Every year, Alibaba has more than 240 events which stores offer special discount, such as Double 11 Global Delight Event, Tmall Thanksgiving Day Event, 1212 Global Discount Event, etc.
Due to the high demand for the UI development in the duration of events, we are required to implement UIs in 3 or 4 days.}


Developers also considered the trade-off between UI performance and its value. 
Since the usage of icon font does not provide business value, it is often in a low priority in industry. 
Even if they knew the benefit of using font, they would not put effort in doing this. 
For instance, D9 explained:

\textit{Although I know the icon font is better compared to icon image, I will not apply this approach in development.
I usually have 3 tasks in a week, such as UI implementation, bug testing, algorithm implementation, etc.
I agree that icon font can improve UI rendering performance and provide better user experience.
% If I do not do this, it will not have any negative effects.
But, the overall functionality will still work without icon font. 
% In contrast, if I do not test the bugs, when it appears, it will have a significant negative impact on the business value.
In contrast, without bug testing, the front-end codes may not work, resulting in significantly impact on the company business.  
And if I do not implement the algorithm, other developers will not be able to apply the API in their development, which will slow down the development speed and delay the product release time.
% Second, I understand that using font can render icon faster, however, it is not the work that I should consider.
% As a UI developer, I mainly focus on how to 100\% exactly implement the UI designs from designers to code.
% The performance testing, efficiency testing, and bug testing should be the work for UI tester.
}

Another example shows the potential gap between industry and individual is that 50\% developers mentioned that they use font to render icons when developing their personal projects, such as homepage, blog, tutorial, etc. 
For example, D2 said,

\textit{When I developed my first personal website, I discovered Font Awesome~\cite{fontawesome}, a font toolkit to render icons by simply adding class description.
Since this is my website, I can design freely according to my preferences.
To quickly develop my website, I used the font in Font Awesome to implement all the icons in my website.
However, it is not applicable in industry.
In industry, every icon is well designed according to the company culture and design specifications. Therefore, it is not suitable to apply widely used icon font resources from online platforms.
In addition, using online icon fonts involves intellectual property (IP) issues which must be avoided in the industry.}

\noindent\fbox{
    \parbox{0.98\textwidth}{
        Despite most of the developers know the benefits of using font to render icons, few of them implement font in practice.
        The icon they used is distinct to the online resources as it comprises company culture and design guidelines. 
        % Therefore, rather than directly using the online resources, developers require effort to convert icon images to font. 
        Therefore, rather than directly using the online resources, developers have to spend extra effort in converting icons to font, which is time-consuming and laborious.
        % However, this process is less valuable in terms of spending a lot of time.
        % However, the process is time-consuming and requires laborious effort.
    }
}

% \begin{tcolorbox}
% \end{tcolorbox}

\subsection{Research Question 3: do developers write descriptions for icons?}
\label{rq2}
% \sidong{工作压力大，更新迭代快，代码的可读性不做要求？}
All of them mentioned that they did write descriptions/comments in their personal projects, such as assignments, homepage, etc.
% Nevertheless, half of developers wrote descriptions in practice, while the other half of them did not. 
% This is because of few practical reasons. 、
However, half of developers did not write descriptions in practice due to the following practical reasons.
% First, because the company requires developers to summarise their work frequently  to record the progress, there are lots of formatted documents for developers to complete. 
\begin{comment}
First, developers have to complete lots of formatted documents required by the company, which are used to record and summarize their work.
Some developers (D1, 2, 5, 9) are tired of writing document, leading to insufficient descriptions in code. 
For example, D8 said,

\textit{We are required to write reports weekly, monthly, quarterly, yearly.
I am poor on writing reports, and this is the major reason that I choose to be a developer.
However, I am still required to documentation in practice.
Compared with solving bugs and implementing codes, I think this task is more challenging.
For each document, I have to spend a lot of time and rack my brains. 
In turns, I spend less effort and time on writing descriptions as it does not affect the outcomes.
}

Some developers use few descriptions in code because they think that the documentation is equivalent to the descriptions.
For instance, D1 said, 

\textit{Since writing weekly report is compulsory, I adopt a combination way of writing report and description to save time.
For weekly report, I write down the contribution, critical thinking and solution.
Then I push the work to git and map it with my weekly report,  which is used as the descriptions/comments of the code.}
\end{comment}
First, since the readability of code is not a mandatory requirement, many developers did not write well-formatted descriptions for code. 
For example, the code in the industry cannot be released as open-source.
As D9 said that \textit{"Since our code can not be released to public, I would not spend too much time on writing comments in code because only a few internal developers would collaborate on my tasks."}
In addition, since updating iteration in the industry is fast, it is not worth to put too much effort in commenting, especially for icons.
For example, D10 said, 
\textit{In the year of 2019, our company developed over 1 million UIs.
Due to the diversity of UIs, few designs are re-implemented and few code are reviewed. Because of the fast updating iteration and low reusing rate, I did not write well-formatted comment, particularly for the images.
I was developing a shopping application which images cover more than half of the UIs.
To develop the large amount of images quickly, I prefer using <img> tag without any alternative description.
}

Second, 80\% developers mentioned that writing a well understood description is a challenging task. 
It requires developers to understand the intention of the icons, while few developers pay attention to the content of the UIs.
For example, D7 explained,

\textit{I agree that the clear descriptions in the code can keep the code readable and “save lives”, while unreasonable descriptions “kill lives”. 
However, it is hard to write a good description. 
Here is the process of how I write the descriptions: 
Firstly, I design a comment for every component, image, ..., based on its characteristic. 
Secondly, I rename and simplify the comments according to practical requirement. 
Thirdly, I check if the comments match the content of UIs or not. 
Then I repeat this process until the deadline.
And obviously, the process is time-consuming and not applicable in the industry.}

Despite the insufficient descriptions in the code may not impede professional developers, it creates a significant cognitive burden for interns and new developers.
For example, D3 said,

\textit{I am a junior student who came to the company for internship.
The first task assigned to me by my leader was to understand the code.
However, I found that most of the code is uncommented, which makes it very difficult for me to understand.
% This potentially leads me not to write the descriptions.
To understand this part of code, I asked more than 5 developers who participated this project.
These uncommented codes negatively influenced my work. 
}


\noindent\fbox{
    \parbox{0.98\textwidth}{
        Developers rarely write descriptions for images, especially for icons, because the loose restriction on code readability makes developers less cared about code descriptions.
        % Most of developers agree with difficulty on thinking a good descriptions, which needs to be simple, concise and well-understood.
        Most of developers agree with difficulty on designing simple, concise and easy-understood  descriptions.
        % The lack of description can adversely affect new employees and lead to inadequate understanding of the code.
        The lack of description can adversely affect novice employees and lead to inadequate understanding of the code.
    }
}

% Developers rarely write descriptions for images, especially for icons, because cumbersome documentation results in insufficient time in comments.

==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/evaluation.tex <==
\section{Experiments}
In this section, we first set up an experiment to analyze the performance of our tool. Then we conduct a pilot user study to evaluate the usefulness of our tool. Furthermore, we demonstrate its usefulness on a large-scale industrial benchmark. 
The goal of our experiments is to answer the following research questions, in terms of accuracy, efficiency and applicability.
\textit{RQ 1: how accurate is our heuristic algorithm in composing icons from design artifacts?}
\textit{RQ 2: how accurate is our model in predicting labels for icon images?}
\textit{RQ 3: how much do our tool increase the efficiency of UI development?}
\textit{RQ 4: what are the developers' opinions on the usability of our tool?}


\subsection{Icon Composition}
\subsubsection{Dataset:}
To evaluate the performance of our heuristic composition algorithm, we compare our automatically generated icon to manually generated ground truth.
To generate the ground truth, we had one author and 10 non-author paid annotators independently label the components in the design artifacts (e.g., the component belongs to \textit{not-icon} or \textit{$icon_x$}, as one artifact may contains multiple icons, we apply $x$ to annotate icon separately).
Each design artifact was labeled by 3 different annotators and the ground truth was generated until an agreement was reached.
All annotators have previous experience designing and implementing icons.
In total, annotators labeled 1,012 real-world design artifacts with 9,883 icons.




\subsubsection{Baselines \& Metrics:}
Since the number of icons in the design artifact is unknown, we set up two widely-used clustering algorithms that do not need to pre-set the number of clusters in advance as baselines, Mean-Shift Clustering~\cite{cheng1995mean} and Density-Based Spatial Clustering of Applications with Noise (DBSCAN)~\cite{ester1996density}.
To further gauge the advantages of our heuristic icon composition algorithm, we compare the icon produced by our correlation metric to each metric individually.
% Specifically, the correlation metric is computed by three factors: attribute, hierarchy, and rendering.

\textit{Mean-Shift:}
Mean-shift is a centroid-based clustering algorithm to detect the close components in the design artifact. 
It works by updating the candidates for the center points as the mean of the points within the sliding window. 

\textit{DBSCAN:}
It is an improvement over the Mean-Shift clustering as it involves a transitivity based chaining-approach to determine whether components are located in a particular cluster, in order to separate clusters of noise and outliers.



\textit{ATTR only:} It composes the icon based on the component's attribute in the artifacts, such as the curve components are merged together as an icon.


\textit{HRCHY only:} As designers may manage all the resources of the icon under a layout folder, we rely on this hierarchical structure information to assemble the icon.


\textit{IOU only:} The rendering of components in the icon are likely intersecting and overlapping to each other, therefore we compose the icon based on measuring the IOU of rendering.


To evaluate the performance, we set up three evaluation metrics, e.g., precision, recall, F1-score.
Precision is the proportion of icons that are correctly composed among all icons in the design artifacts.
Recall is the proportion of icons that are correctly composed among all composed components (e.g., \textit{$icon_x$} and \textit{not-icon}).
F1-score is the harmonic mean of precision and recall, which combine both of the two metrics above.



\begin{table}[t!]
    \centering
    \begin{tabular}{l|cc|ccc|c}
    \toprule
    \bf{Method} & Mean-Shift & DBSCAN & ATTR only & HRCHY only & IOU only & Our \\
    \hline
    \bf{Precision} & 40.16\% & 55.54\% & 27.10\% & 3.23\% & 45.40\% & \bf{76.50\%} \\
    \hline
    \bf{Recall} & 51.91\% & 73.34\% & 35.20\% & 6.25\% & 62.51\% & \bf{81.25\%} \\
    \hline
    \bf{F1-score} & 45.28\% & 63.21\% & 30.62\% & 4.26\% & 52.59\% & \bf{78.80\%} \\
    \bottomrule
    \end{tabular}
    \caption{Performance comparison for icon composition.}
    \label{tab:compositionResult}
\end{table}



\begin{figure}
	\centering
	\subfigure[Compared to \textit{ATTR only}, our algorithm can compose icon with different attributes (bitmap and path).]{
		\includegraphics[width = 0.3\textwidth]{figs/example1_1.png}
		\label{fig:example1}}
	\hfill
	\subfigure[Compared to \textit{HRCHY only}, our algorithm can compose icon with different hierarchies ("Oval" not in the layout folder).]{
		\includegraphics[width = 0.3\textwidth]{figs/example2_1.png}
		\label{fig:example2}}	
	\hfill
	\subfigure[Compared to \textit{IOU only}, our algorithm can compose icon with no intersection (shapes are widely spaced).]{
		\includegraphics[width = 0.3\textwidth]{figs/example3_1.png}
		\label{fig:example3}}	
	\caption{The results of our icon composition algorithm. The top represents the design artifact, and the bottom represents the clustering steps.}
	\label{fig:iconresult}
\end{figure}




\subsubsection{Results:}
Table~\ref{tab:compositionResult} shows the performance of all methods.
The centroid-based clustering algorithm can only achieve 45.28\% and 63.21\% F1-score, for \textit{Mean-Shift} and \textit{DBSCAN} respectively.
The issues with these baselines are that they are designed for large and dense data, such as natural disasters, stations, etc.
However, different from those data, the number of components in design artifacts is relatively small.
The performance of our algorithm is much better than that of other correlation baselines, e.g., 31.1\%, 18.74\%, 26.21 boost in precision, recall, and F1-score compared with the best correlation baseline (\textit{IOU only}).
Relying only on hierarchical structure information (\textit{HRCHY only}) yields poor performance in all metrics, 3.23\%, 6.25\%, and 4.26\% respectively compared to the ground truth.
This is because that many designers follow their own design styles which highly differ from each other, and some of their design miss the rigid layout information. 
\textit{ATTR only} yields an average F1-score of 30.62\%, which is better than the F1-score of \textit{HRCHY only}, indicating that the attribute of components provides better information for icon composition as designers tend to use consistent attributes for icon designs.
\textit{IOU only} yields the best performance among all baselines with the average F1-score to 52.59\%, indicating that the icons are normally composed by several intersecting components.
Fig~\ref{fig:iconresult} shows some results of icon composition by our heuristic algorithm. 
It shows that our algorithm can help cluster the components with different attributes (e.g., bitmaps and path for the first icon), different hierarchies (e.g,  "Oval" component is not in the layout for the second icon), and no intersection (e.g., the components of icon have spacing for the third icon).


% Although our heuristic correlation metric that combines attribute, hierarchy, and rendering, greatly improves the performance of icon composition, we still make mistakes for some icons.

To identify the common causes of errors, we further manually check the wrong composition cases in the test dataset. 
According to our observation, we found two main reasons.
First, the components of icons are widely spaced, such as, three separated waves for "wifi", three horizontal lines for "menu", several lines from low to high for "signal", etc.
In addition, designers may depict some effects around the icon, such as, the ripple effect on a hand for "tap", the shiny effect on a bulb for "light", etc.
The wide space between components decreases the correlation value of IOU, resulting in poor clustering.
Second, some designers place icon and text in the same hierarchy to depict an image button, for example, a folder consists of icon components, text components, button border, etc., causing our algorithm to aggregate an image button, rather than an icon.









\subsection{Icon Prediction}
\subsubsection{Dataset:}
We leveraged the categorization during the creation of the semantic vocabulary (in Table~\ref{tab:categorization}), and corresponding icons and attached labels as the training data.
The foundation of the deep learning model is the big data, so we only selected categories with frequency larger than 300 for training the model.
Therefore, there are 100 categories left with the number of icons ranging from 311 to 589. 
Given all the data assigned to each label, we randomly split these 41k icons into train/validation/test dataset with a ratio of 8:1:1 (33K:4K:4k).
To avoid the bias of of “seen samples” across training, validation and testing, we performed 5-fold cross-validation.

\subsubsection{Baselines:}
We set up several basic machine-learning baselines including the feature extraction (e.g., color histogram~\cite{wang2010robust}, scale-invariant feature transform~\cite{lowe1999object}) with machine-learning classifiers (e.g., decision tree~\cite{quinlan1983learning}, SVM~\cite{cortes1995support}).
% Color histogram (Histo) is a simple image feature that represents the distribution of colors in each RGB (red, green, blue) channel.
% It has been widely used for image indexing and image retrieval~\cite{jain1996image, han2002fuzzy, hafner1995efficient}.
% The scale-invariant feature transform (SIFT) is an advanced image feature which locates keypoints in images and use the local features of the keypoints to represent images.
% Based on these hand-crafted features, we adopted the support vector machine (SVM) and decision tree (DT) as the classifiers.
Apart from these conventional machine learning based baselines, we also set up several derivations of state-of-the-art deep learning models as baselines to test the importance of different inputs of our approach including backbones (ResNet~\cite{he2016deep}, VGG~\cite{simonyan2014very}, MobileNet~\cite{sandler2018mobilenetv2}), different input channels (RGB, RGBA).  
The training and testing configurations for these baselines were the same.

\begin{table}[t!]
    \centering
    \footnotesize
    \begin{tabular}{l|cccc|cccc}
    \toprule
    \bf{Method} & \specialcell{\bf{Histo} \\ \bf{+SVM}} & \specialcell{\bf{Histo} \\ \bf{+DT}} & \specialcell{\bf{SIFT} \\ \bf{+SVM}} & \specialcell{\bf{SIFT} \\ \bf{+DT}} & \bf{ResNet-50} & \bf{VGG-16} & \specialcell{\bf{MobileNetV2} \\ \bf{(RGBA)}} & \specialcell{\bf{MobileNetV2} \\ \bf{(RGB)}}\\
    \midrule
    \bf{Accuracy} & 0.5657 & 0.3267 & 0.5806 & 0.4686 & \bf{0.8839} & 0.8764 & 0.8348 & 0.8772 \\
    \hline
    \bf{Time (ms)} & 0.103 & 0.152 & 1.702 & 1.941 & 26.535 & 27.282 & 17.567 & \bf{17.485} \\
    \bottomrule
    \end{tabular}
    \caption{Label classification accuracy and time estimation in different methods.}
    \label{tab:predictresultTable}
    % \vspace{-1cm}
\end{table}




\subsubsection{Results:}
\label{prediction_result}
As we trained a classifier to predict label for icon, we adopted the accuracy as the evaluation metric for the model, illustrated in Table~\ref{tab:predictresultTable}.
% The detailed result is illustrated in Table~\ref{tab:predictresultTable}.
The traditional machine learning method based on the human-crafted features can only achieve about 0.6 average accuracy.
Deep learning models perform much better than the best old fashioned methods, i.e., with the 0.3033, 0.29712, 0.2958 increase for ResNet-50, VGG-16, and MobileNetV2 respectively.
Although ResNet model performs the best in icon classification task, it requires relatively long time for prediction (26.535ms per icon) which strongly violates the performance of UI rendering (16ms) as we aim to deploy into an online platform (\textit{Imgcook}).
In contrast, our model MobileNet is nearly as accurate as ResNet with a performance lag of 0.67\%, while being 34.1\% faster.
And also, we find that the increase of a fourth alpha channel (RGBA) decreases the accuracy from 0.8772 to 0.8348, due to two main reasons.
% three-channel RGB color model supplemented with a fourth alpha channel.
% To identify the causes of the decrease, we then further manually check the true-false predictions in the test dataset, i.e., predicting true in RGB while false in RGBA. 
% According to our observation, there are two main reasons leading to the decrease. 
First, the result shows that the model with RGB input has a loss value of 0.7844 at epoch 200, which is better than the model with RGBA (0.9231). This is because the supplemented channel greatly increases the parameters of the model, which leads to a decline in the ability of gradient training at the same epochs.
Second, based on the principle of optics, the fourth alpha channel does not reflect the morphological characteristics of the image. It is used to reduce information of other three channels by adjusting their color/degree, causing less information captured through training process.


\subsection{User Study}


\begin{table*}[t!]
\caption{Examples of development for icons in \textbf{E}xperimental and \textbf{C}ontrol groups.}
% $E$ denotes the code generated by our method, $C$ denotes the code developed by developers.
\centering
% \footnotesize
\begin{tabular}{p{0.3\linewidth}|p{0.05\linewidth}p{0.5\linewidth}}
    \toprule
    % \multicolumn{1}{c|}{\bf{Icon Image}} &  \multicolumn{2}{c}{\bf{Output Code}} \\
    % \midrule
    \multirow{4}{*}{\begin{minipage}[t]{2em}\centering\includegraphics[width=1.75in]{figs/userstudyimplement1.jpg}\end{minipage}} & \bf{E} & \small{<i class="icon-left red"></i>} \\ \cmidrule{2-3}
    & \bf{C1} & \small{<img src="8E431911-61BB-4A19-8C01.svg"/>} \\
    \cmidrule{2-3}
    & \bf{C2} & \small{<img src="next-icon-design.svg" alt="next" width="100\%"/>} \\
    \cmidrule{2-3}
    & \bf{C3} & \small{<div style="background-image: url('8E431911-61BB-4A19-8C01.svg');"></div>} \\
    \midrule
    \multirow{4}{*}{\begin{minipage}[t]{2em}\centering\includegraphics[width=1.65in]{figs/userstudyimplement2.jpg}\end{minipage}} & \bf{E} & \small{<i class="icon-information white"></i>} \\ \cmidrule{2-3}
    & \bf{C1} & \small{\begin{tabular}[c]{@{}l@{}}\textless{}svg class="icon" aria-hidden="true"\textgreater\\   \hspace{0.5cm} \textless{}use xlink:url="icon-information"\textgreater{}\textless{}/use\textgreater\\ \textless{}/svg\textgreater{}\end{tabular}} \\
    \cmidrule{2-3}
    & \bf{C2} & \small{<a style="background-image: url('q\&a.svg'); width: 100\%; height:100\%;" class="help-icon"></a>} \\
    \cmidrule{2-3}
    & \bf{C3} & \small{<a class="svg-icon-info" href="\#"><SvgIcon name="white"></a>} \\
    \bottomrule
\end{tabular}
\label{tab:icon_development}
\end{table*}

% \begin{table}[ht]
% \begin{minipage}[b]{0.4\linewidth}
%     \centering 
% 	\includegraphics[width=0.9\linewidth]{figs/Boxplot.pdf}  
% 	\caption{Distribution of time measurements by human development (Control) and the model (Experiment).} 
% 	\label{fig:time}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%     \bf{Measures} & \bf{Control} & \bf{Experimental} \\
%     \midrule
%     Time & 17.39s & 6.05s \\
%     Readable & 2.8 & 4.16$^{**}$ \\
%     Acceptable & 3.96 & 4.7$^*$ \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:score_Table}
%     \caption{The comparison of the experiment and control groups. $^*$denotes $p<$ 0.01, $^{**}$denotes $p<$ 0.05.}
% \end{minipage}
% \end{table}


\subsubsection{Procedures for User Study}
10 developers (generators), all proficient in UI development and have at least 1-year experience, were recruited for this study.
We randomly selected five icons from the real-life UI designs and asked each generator to develop them.
To guarantee the generators can objectively develop the icons, we asked whether they have prior knowledge on the icons (such as development experience, design experience, etc.).
The time of the development were recorded.
To be fair, generators did not know we were recording the time as the time pressure may affect their development (in quality, speed, etc.)~\cite{austin2001effects,mantyla2014time}.
We set the manual development as the control group.
Then, we also asked them to develop five other icons with the help of our tool which not only automatically convert the image to font, but also provide the description (predicted label and color).
We called this the experimental group.
The detailed developments of two groups for icons are shown in Table~\ref{tab:icon_development}. 

We then recruited another 10 developers (evaluators), and each of them was assigned the developments from two control groups and one experimental group.
Note that they did not know which one if from the experimental or control group, and for each icon, we randomly shuffled the order of candidates to avoid potential bias.
Given each development, they individually marked it as readable or not in five-point likert scale (1:not readable at all and 5:strongly readable).
To evaluate the performance of usability, we also asked evaluators to rate how likely they would like to use the development in practice (Acceptable).
The measurement is also in five-point scale.

% \begin{figure}  
% 	\centering 
% 	\includesvg[width=\linewidth]{figs/userstudyresult.svg}  
% 	\caption{The comparison of the experiment and control groups. $^*$denotes $p<$ 0.01, $^{**}$denotes $p<$ 0.05.} 
% 	\label{fig:time}
% \end{figure}

\begin{figure}
    \centering
    \begin{minipage}{.65\textwidth}
        \centering
        \includegraphics[height=1.7cm]{figs/userstudyresult.png}
        \caption{The comparison of Experimental and Control groups. $^*$denotes $p<$ 0.01, $^{**}$denotes $p<$ 0.05.}
        \label{fig:time}
    \end{minipage}%
    \hfill
    \begin{minipage}{.28\textwidth}
        \centering
        \includegraphics[height=1.8cm]{figs/serendipitous.jpg}
        \caption{The icon description varies by context.}
        \label{fig:serendipitous}
    \end{minipage}
\end{figure}


% \begin{table}[ht]
% \caption{The comparison of the experiment and control groups. $^*$denotes $p<$ 0.01, $^{**}$denotes $p<$ 0.05.}
% \centering
% \begin{tabular}{lcc}
%     \toprule
%     \bf{Measures} & \bf{Control} & \bf{Experimental} \\
%     \midrule
%     Time (s) & 17.39 & 6.05$^*$ \\
%     Readable & 2.8 & 4.16$^*$ \\
%     Acceptable & 3.96 & 4.7$^{**}$ \\
%     \bottomrule
% \end{tabular}
% \label{tab:score_Table}
% \end{table}


\subsubsection{Results:}
\label{user_study_result}
Box plot in Fig~\ref{fig:time} shows that the time spent on the development of icons in the experimental group is much shorter than that in the control group (with an average of 6.05s versus 17.39s, saving 65.2\% of time).
That is the biggest strength of our tool i.e., developers can quickly develop an icon by providing descriptions and a font pattern.
On average, the overall readability ratings for the experiment group is 4.16, which are significantly higher (48.5\%) than the control group (2.8) in Fig~\ref{fig:time}. 
Most developers admit that our tool can provide more acceptable results for them.
In other words, 94\% (4.7/5.0) of developers hope to develop the icons with the help of our tool in their real development environment compared to 3.96 in the control group.
To understand the significance of the differences, we carry out the Mann-Whitney U test~\cite{fay2010wilcoxon} (specifically designed for small samples) on the readability and acceptability ratings between the experiment and the control group respectively. 
The test results suggest that our tool does significantly outperform the baseline in term of these metrics with $p < 0.01$ or $p < 0.05$.
% Although by no means conclusive, the user study provides initial evidence of the usefulness of our tool for enhancing the performance of UI development.
% The results show that \textit{Auto-Icon} can surpass control group by a large margin.

For some icons, the developer gives very low acceptability score to the labels. 
According to our observation and further survey, we summarise two reasons accounting for those bad cases. 
(1) Albeit the good performance of our model, we still make wrong predictions for serendipitous icons. Based on the context of icon, the same icon can have different meaning.
For example, the icon in Fig~\ref{fig:serendipitous} represents the meaning of "information" in the common case, but consider the text on the right, the meaning of the icon should be "glossary"/"dictionary". 
% (2) Developers see high potential in being able to automatically convert icons to fonts to render UI faster.
(2) Developers admit the usefulness of converting images to font for providing faster rendering speed.
However, they also point out the limitation of replacing image with font.
Font is not fully compatible in all browsers and devices. One developer mentioned that they need to make sure that the development works on old devices, in which they usually need to give up latest efficient methods, such as iconfont. 
% \sidong{any more suggest?}


\subsection{Industrial Usage}
We cooperate our tool with the \textit{Imgcook} platform\cite{imgcook} developed by Alibaba, an intelligent tool to automatically generate front-end codes from UI design files.
\textit{Imgcook} has attracted a lot of attention in the community which has a large user base (15k) and generates over 40k UIs.
\tool is integrated with the internal automated code generation process and is triggered whenever the design files contain an icon. 

% Time metric is an important indicator to measure the efficiency of our method, however, it is hard to control variables and conduct reasonable experiments in \textit{Imgcook}, because developers who are proficient in \textit{Imgcook} will spend less time on development.
% To address this problem, we set up a code review metric for measuring the code modification for icon designs. 
% If developers make fewer changes on code, we then assume that our method help them save time and effort.
% Note that the code modification contains multiple contents, such as text, button, etc, we only measure the modification if the object is icon.
% We adopt a case-insensitive BLEU (BiLingual Evaluation Understudy)~\cite{?} metric to evaluate the preservation of code. BLEU is an automatic evaluation metric widely used in code difference studies. It calculates the similarity of machine-generated code and human-modified reference code (i.e., ground truth), which is calculated as:

In order to evaluate the usability of our tool, we set up a code review metric for measuring the code modification for icons. 
Note that the code modification contains multiple contents, such as text, button, etc, we only measure the modification if the object is icon to reduce the potential bias.
We adopt a case-insensitive BLEU (BiLingual Evaluation Understudy)~\cite{papineni2002bleu} as the metric to evaluate the preservation of code. BLEU is an automatic evaluation metric widely used in code difference studies. It calculates the similarity of machine-generated code and human-modified reference code (i.e., ground truth) as
\(BLEU = BP * exp(\sum_{N}^{n=1} w_{n}logp_{n})\)
% \begin{equation}
% BLEU = BP * exp(\sum_{N}^{n=1} w_{n}logp_{n})
% \end{equation}
where $p_{n}$ denotes the precision, i.e., the ratio of length n token sequences generated by our method are also present in the ground-truth; $w_{n}$ denotes the weight of different length of n-gram summing to one; $BP$ is 1 if c > r, otherwise $e^{(1-r/c)}$ where c is the length of machine-generated sequences and r is the length of ground-truth.
A high BLEU score indicates less modification in the code review.


% \begin{figure}  
% 	\centering 
% 	\includegraphics[width=\linewidth]{figs/badcase.png}  
% 	\caption{An example of code modification.} 
% 	\label{fig:badcase}
% \end{figure}

We run the experiment in \textit{Imgcook} with 6,844 icons in 2,031 UIs from August 20, 2020 to September 20, 2020.
% Figure~\ref{?} plots the distribution of elements of each category in the UIs and shows the importance of icon designs in the real world UI development, accounting for 20\% (4,753) of the total number.
Among all the testing UI developments, the generated code for icon reaches 84\% BLEU score, which means that most of the code is used directly without any modification. It demonstrates the high usability of \tool in practice. 
% It also confirms that our tool help developers save time and effort if they make fewer changes on code.
Based on the inspection results, we categorize the modification into four categories.
Two reasons are discussed in the Section~\ref{user_study_result}, in terms of wrong prediction and compatibility concern.
There are another two modifications mainly due to industrial practice. 
First, in order to maintain the consistency of company's coding experience, some developers modify to a prescribed naming/rendering method, for example, packing the icon of "icon-camera" to a <Icon-Camera> tag.
% Second, UI changes in practice dynamically. 
Second, UI dynamically changes in practice.
Once an element in the UI is changed, the attribute of icon may change, such as color and font size.



% To investigate how much our method improve the efficiency, we compared the development time of Imgcook with and without our method. The result of the comparison is shown in Figure~\ref{?}.
% We found that the average time of development is declining every month.
% It is consistent with human perception, as users become more proficient in using \textit{Imgcook} without spending less effort of learning it.
% To avoid the bias and establish fair experiment, we target the top 20 active developers which regularly (at least five development comments weekly).
% All of them have used \textit{Imgcook} for at least one year and have a wealth of expertise.
% Figure~\ref{?} shows the time estimation of them developing UI with and without our method.
% We can see that the average developing time of using our method was slightly shorter than that without our method.
% The reason for this difference is the presence of a potential manual step in icon development.
% While the developers develop the icon designs in UI, our method automatically generates the applicable codes with readable descriptions which saves time and effort.


\noindent\fbox{
    \parbox{0.98\textwidth}{
        Overall, our method achieves 78.8\% F1-score in the icon composition from design artifacts (RQ1), and 87.7\% accuracy in the label prediction for icons (RQ2).
        % Of the survey of 10 developers, we improve the efficiency of developing time and code readability by 65.2\% and 48.5\%, respectively (RQ2).
        In the survey of 10 developers, we improve the efficiency of developing time and code readability by 65.2\% and 48.5\%, respectively (RQ3).
        The majority (4.7/5.0) of the interviewed developers acknowledges the usability of the generated code for icon by our method, and it is further confirmed in the practice of \textit{Imgcook} with 84\% BLEU score (RQ4).
    }
}


==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/introduction.tex <==
\section{Introduction}
% There are series of elements that make up an user interface (UI), such as text, colors, images, illustrations, etc. 
A user interface (UI) consists of series of elements, such as text, colors, images, widgets, etc.
% Some of these elements are icons, which are used in a variety of UIs with different styles.
% To enhance the diversity of UIs, icons are widely used.
Designers are constantly focusing on icons as they are highly functional in a user interface~\cite{koutsourelakis2010icons,black2017icons,islam2015exploring,malik2017sustainable}.
One of the biggest benefits of icons is that they can be universal. 
% When you add a red “X” to your user interface design, just about every single user will understand that clicking that icon makes whatever it is on disappear.
For instance, by adding a red “X” icon to your user interface design, users are informed that clicking this icon leads to the closure of a component.
Furthermore, icons can make UIs look more engaging. For example, instead of using basic bullets or drop-downs filled with words, a themed group of icons can capture instant attention from users.
Consequently, icons become an elegant yet efficient way to communicate with and help guide user through experience. 

Despite of all these benefits, icons have three fundamental limitations in the day-to-day development environment, in terms of \textit{transition gap}, \textit{rendering speed} and \textit{code accessibility}.
First, it is a challenging task for developers to implement icons from the design artifacts as many designers follow their own design styles which are highly differ from each other.
% Some of their design miss the rigid layout information. 
% For example, they may annotate that some components are in one group while not doing so for other components.
For example, some of them design an icon with many small components, though just one combined image in the icon implementation for optimizing the network traffic and caching.
Such gap adds the complexity and effort for developers to preprocess the design draft before icon implementation.
Second, to ensure a smooth user interaction, UI should be rendered in under 16ms~\cite{gomez2016mining,slowrendering,slowrendering2}, while icon implemented as an image faces the slow rendering problem, due to image download speed, image loading efficiency, etc.
These issues will directly affect the quality of the product and user experience, requiring more effort from developers to develop an advanced method to overcome the problem.
Third, in the process of UI implementation, many developers directly import the icon resources from the design artifacts without considering the meaning of the content, resulting in poor description/comment during coding.
% For example, \sidong{Figure~\ref{?}} shows some icons in the UIs and its corresponding codes. 
Different codes render the same visual effect to users, while it is different for developers to develop and maintain.
A non-descriptive code increases the complexity and effort required to developers as they need to look at the associated location of the UI to understand the meaning of the code.
% The rendered icons look the same for the users, while the code is undescriptive for the developers, particularly difficult for further development and maintain.
% Since developers need to look at the associated location of the UI to understand the meaning of the code, increasing the complexity and effort required to developers.
\begin{comment}
Therefore, we investigate the impact of these requirements in practice, resulting in two research questions: \textit{1) do developers implement icon design in font or image?} \textit{2) do developers write descriptions for icon design?}
To answer the research questions, we conduct an preliminary study with 12 professional developers
We found that although developers acknowledge the benefit of icon font, they still to use images with little/no descriptive text to implement icon designs due to the huge pressure of real world development environment. 
\end{comment}
% Moreover, we interview \sidong{?} professional developers who have developed UIs for at least a year.
% We investigate their process of UI development and their impact.
% \sidong{We find that }
% We found that users’ configurations and the rationale behind their configurations evolve over time due to changing social contexts. Additionally, users’ configurations of audience control have various impacts on their online information disclosure and social interactions with others, which in turn prompts them to adjust their configurations and their rationales for these configurations.

This challenge motivates us to develop a proactive tool to address the existing UI development limitations and improve the efficiency and accessibility of code.
% which automatically convert an icon image to an icon font with label descriptions,
Our tool, \tool involves four main features.
First, to bridge the conceptual gap between icon design and icon implementation, we propose a heuristic machine learning technique to automated agglomerate the scattered icon components into clusters.
The component clusters can then be composed to icon images, which can be applied in various downstream tasks related to improving the rendering efficiency (i.e., icon font, css clipping) and code accessibility (i.e., description, color).
Second, to meet the requirement of efficient rendering, we develop an automated technique to convert icon image to icon font, which is a typeface font.
Once the font is loaded, the icon will be rendered immediately without downloading the image resources, thereby reducing HTTP requests and improving the rendering speed. Icon font can further optimize the performance of rendering by adopting HTML5 offline storage.
Besides, icon font has other potential attributes that can facilitate UI development, such as easy to use (i.e., use the CSS's @fontface attribute to load the font), flexible (i.e., capable to change color, lossless scale), etc.
% This tool is flexible (i.e., capable to change color, lossless scale, etc.), easy to use (i.e., use the CSS's @fontface attribute to load the font), able to improve the load efficiency (i.e., font is loaded before image, so there is no need to worry about the problem of poor image loading issue).
Third, understanding the meaning of icons is a challenging problem.
There are numerous types of icons in the UIs. Icons representing the same meaning can have different styles and can be presented in different scales as shown in Table~\ref{tab:categorization}. Also, icons are often not co-located with texts explaining their meaning, making it difficult to understand from the context. 
In order to offer an easy access for developers to develop through understanding the meaning of icons, we collect 100k icons from existing icon sharing website Alibaba Iconfont~\cite{iconfont} - each associating with a label described by designer.
By analyzing the icons and labels, we construct 100 categories, such as "left", "pay", "calendar", "house", etc. 
We then train a deep learning classification model to predict the category of the icon as its description.
The experiments demonstrate that our model with the average accuracy as 0.87 in an efficient classification speed as 17.48ms, outperforms the other deep learning based models and computer vision based methods.
Third, to provide more accessibility to developers on the description of icon images, we also detect the primary color of icons by adopting HSV color space~\cite{sural2002segmentation}.
We refer to our mechanism tool \tool to build an intelligent support for developers in the real context of UI development, assisting developing standardized and efficient code.

To demonstrate the usefulness of \tool, we carry out an user study to show if our tool for automatically converting an icon to a font with label descriptions can help provide more knowledge on code accessibility and accelerate UI development for developers.
After analyzing ten professional developers' feedback with all positive responses on our mechanism tool and we find that the code for icon generated by our tool can achieve better readability compared with the code manually written by professional developers.
Besides, \tool has been implemented and deployed in Alibaba \textit{Imgcook} platform. The results demonstrates that our tool provides 84\% usable code for icon designs in a realistic development situations.
% first conduct an experiment on the efficiency of rendering font compared to other rendering ways.
% We also carry out a user study to show if our model for adding icon description can help provide more knowledge on code accessibility for developers. 
% After analyzing \sidong{ten} professional developers' feedback, they are positive about our mechanism, and could envision intriguing uses of the mechanism in realistic development situations.
Our contributions can be summarized below:
\begin{itemize}
    \item We identify the fundamental limitations of existing UI development of icon images.
    The informal interviews with professional developers also confirm these issues qualitatively.
    \item To bridge the gap between icon design and icon implementation, we develop a machine-learning based technique to compose the components of icon in the design artifact.
    \item Based on the emerging 100 icon categories, we develop deep-learning and computer-vision based techniques for specifically converting icon to font with label describing its meaning and color to provide developers understand knowledge of code.
    \item We conduct large-scale experiments to evaluate the performance of our tool \tool and shows that our tool achieves good accuracy compared with baselines.
    The evaluation conducted with developers and tested on the real-world development platform demonstrates the usefulness of our tool.
    \item We contribute to the community by offering intelligent support for developers to efficiently implement icon designs comply with code standardization.
\end{itemize}

% We will further elaborate these knowledge discovery in the real UI development environment with detailed examples in Section~\ref{?}.


% Due to small screens of smartphones, icons are often not co-located with texts that explain their intents. As exemplified by Figure 1b, Google Map uses the icon shown in red square to center the map to the user’s current location, without any text around the button. Second, some icons are embedded with text, referred to as text icons. For example, the third button from the top shown in Figure 1c indicates that the app will access users’ GPS data. The diversified colors and opacities in fonts and backgrounds (e.g., ghost button [13]) make it difficult to directly apply Optical Character Recognition (OCR) [14], which works best for icons having black texts and white backgrounds.



% With \sidong{million} of real-world design drafts (i.e., PSD, Sketch, etc.) collected from industry - each comprising multiple icon designs of human creativity and aesthetics - these drafts provide an opportunity to learn about the icon usage in practice and understand the intentions of icons on a truly massive scale, even though the icons in the design drafts are not created for the purpose of knowledge discovery.
% However, collecting and inspecting these design drafts in an ad-hoc fashion cannot effectively exploit this gold mine of icon design resources. 
% This paper presents a pipeline to address the described limitations.
% We refer to our pipeline to build an intelligent support for developers in the real context of UI development.

% We first develop an automated technique to convert icon image to icon font, which is a typeface font.
% It is flexible to use (i.e., capable to change color, lossless scale, etc.), easy to use (i.e., use the CSS's @fontface attribute to load the font), provides efficient and fast-loading way (i.e., font is loaded before image, so there is no need to worry about the problem of poor image loading issue).
% Second, in order to address the problem of 
% we collect \sidong{?} icons of \sidong{?} practical UI design drafts and based on the collected design drafts we build a deep learning model to classify the icon.








% To maintain this functionality, it’s important to reduce cognitive load on users by employing icons sparingly and strategically throughout your designs.







% The fundamental mission of an icon is to offer, without distracting, specific visual information. In order to successfully perform this mission, an icon must have a series of characteristics, among which the following stand out:

==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/relatedwork.tex <==
\section{Related Works}
% Our work is problem driven, rather than approach driven. As our study is to support developers with UI rendering and code accessibility intelligently, we are introducing related work in these two aspects.


\subsection{Transition Gap}
UI design and implementation require different mindset and expertise. 
The former is performed by user experience designers and architects via design tools (e.g., Sketch~\cite{sketch}, Photoshop~\cite{ps}), while the latter performed by developers via development tools (e.g., Android Studio~\cite{androidstudio}, Xcode~\cite{xcode}). 
% Our work lowers the transition barrier from UI design artifacts to UI implementation.
Existing researches well support these two phases respectively~\cite{lee2020guicomp, yang2021uis, chen2021should, todi2021conversations, bunian2021vins, zhang2021screen, ang2021learning,feng2021auto}.
For example, Li et al.~\cite{li2021screen2vec} provide a holistic representation of UI to help designers quickly build up a realistic understanding of the design space for an app feature and get design inspirations from existing UI designs.
But few of them support effective transition from UI design artifacts to UI implementation.


Supporting this transition is challenging due to the gap between designers and developers and the complexity of design artifacts (see Fig~\ref{fig:iconexample}).
Some researches lower the transition gap by translating UI screenshots into UI implementation~\cite{chen2018ui,moran2018machine,sketch2codemicrosoft,sketch2codeairbnb, chen2019storydroid,wu2021screen}.
Nguyn et al.~\cite{nguyen2015reverse} follow the mobile specific heuristics and adopt hybrid method based on Optical Character Recognition (OCR) and image processing to generate a static code from UI screenshots.
Pix2Code~\cite{beltramelli2018pix2code} adopts an iterative encoder/decoder deep learning model consisting of a CNN for extracting UI screenshots features, and a LSTM decoder for generating the UI code tokens.
However, these works are unclear if the UI implementations are realistic or useful from a developer’s point of view, as the implementation of the approaches are only validated on a small set of synthetically UI screenshots.
It is difficult to judge how well the approaches would perform on real UI screenshots. 
In contrast, \tool is tailored for the design artifact driven development practice, and is aimed at solving real-world UI development challenges, such as developers requiring manual effort to compose the icon from scattered components in the design artifact.
There has also been both commercial and academic work related to design artifact driven development for creating high-fidelity design artifacts~\cite{fluidui, mockup, proto}, deploying real-device prototype environments~\cite{meskens2009plug,meskens2009shortening}, and verifying design violations~\cite{moran2018automated}.
However, such tools and approaches tend to either impose too many restrictions on designers or do not allow for direct creation of code, thus the icon composition problem still persists in practice.
To address this, we adopt a machine-learning approach to automatically agglomerate the scattered icon components into clusters through heuristic correlation coefficient to bridge the gap between icon design and icon implementation.


% In addition to the engineering challenges associated with building
% an approach to detect presentation failures in the mobile domain
% (e.g., collection and processing of GUI-related data) Gvt is the first
% approach to leverage metadata from software mock-up artifacts
% (e.g., Marketch) to perform GC matching based upon the spatial
% information collected from both mock-ups and dynamic application
% screens, allowing for precise detection of the different types of DVs
% delineated in our industrial DV taxonomy.










% In contrast, we conduct an informal interview with professional developers to identify the gap between designers and developers in practice and this gap points to a more prominent problem, that is developers require manual effort to compose icon from scattered components in the design artifact.
% % To ease the burden of use for developers,
% We then adopt a machine-learning approach to automatically agglomerate the scattered icon components into clusters through heuristic correlation coefficient to lower the transition barriers between icon design and icon implementation.






\subsection{UI Rendering}
% An important step in UI development is measuring the performance.
Ensuring fast rendering speed is an essential part in UI development, since slow rendering creates poor user experience.
% \suyu{Ensuring fast rendering speed is an essential part in UI development, since slow rendering results in poor user experience.
% }
% Slow rendering creates a very bad user experience.
Many studies focus on improving rendering speed via reducing bugs~\cite{carette2017investigating,li2019characterizing,nejati2016depth,huang2017shuffledog,rosen2017push}.
In contrast, we focus on analyzing image displaying performance in UI rendering.
There are a few related works in this domain.
For example, Systrace~\cite{systrace} is a tool that allows developers to collect precise timing information about UI rendering on devices. 
However, it does not provide any suggestions for improvement.
To address this problem, many studies introduce reliable approaches to improve rendering efficiency such as image resizing based on pattern-based analysis~\cite{liu2014characterizing}, a manual image resource management based on resource leakage analysis~\cite{wu2016light}.
Gao et al.~\cite{gao2017every} implement a system called DRAW which aims to reveal UI performance problems in an application such as excessive overdraw and slow image components detection. 
With the suggestion of the image displaying performance analysis by DRAW, developers can manually improve the rendering performance of slow image displaying.
While these works offer image management suggestions to developers to achieve better rendering performance, they still need to be improved manually.
In contrast, we propose an image conversion technology based on computer vision and graphic algorithms to convert icons into font types for achieving faster UI rendering.


\subsection{Code Accessibility}
% Computer, mobile and wearable devices are used in people's daily life.
Digital devices such as computer, mobile phone and tablets are widely used.
% You’ll be astonished at the myriad of devices and apps in your life that are packed with bits of code.
% Consisted with pieces of code, various apps are developed to improve the quality of our life.
% There are many research works for ensuring the quality of apps~\cite{butler2010android, fu2013people, hecht2015tracking}, most of them are investigating the apps’ functional and non-functional properties like compatibility~\cite{wei2016taming}, performance~\cite{linares2015developers,zhao2016novel}, energy-efficiency~\cite{banerjee2016debugging,banerjee2016automated}, GUI design~\cite{chen2019gallery, chen2019storydroid}, GUI animation linting~\cite{zhao2020seenomaly}, localization~\cite{wang2019domain} and privacy and security~\cite{chen2019gui,chen2018automated,dehling2015exploring,feng2019mobidroid,yuan2016droiddetector}.
To ensure the quality of software, many research works have been conducted~\cite{butler2010android, fu2013people, liu2022guided}.
Most of these works focus on the functionality and usability of apps such as GUI design~\cite{chen2019gallery,feng2022gallery, chen2019storydroid,chen2020object,xie2020uied,liu2020owl,zhao2021guigan}, GUI animation linting~\cite{zhao2020seenomaly,zhao2019actionnet}, localization~\cite{wang2019domain,feng2021gifdroid,xie2020uied}, privacy and security~\cite{chen2019gui,chen2018automated,dehling2015exploring,feng2019mobidroid}, and performance~\cite{linares2015developers,zhao2016novel}.
% Few of them are studying the accessibility issues.
Few research works are related to accessibility issues.
Some works in Human-Computer Interaction area have explored the accessibility issues of mobile apps~\cite{ yan2019current,wang2012measurement,mora2017comprehensive,king2016government,chen2020unblind}.
% In Human-Computer Interaction area, some works investigate the accessibility issues in mobile apps~\cite{park2014toward, yan2019current,wang2012measurement,mora2017comprehensive,king2016government}.
% Although they explore different accessibility issues, the lack of descriptions for image-based components in the UI has been commonly explicitly noted as a significant problem in these works.
In these work, the lack of description in image-based components in UI is commonly regarded as an important accessibility issue.
% For example, Ross et al.~\cite{ross2018examining} examine the icon image labeling in the Android apps, and they specify some common labeling issues within the app. 
% Different from their works, our study includes not only the practical analysis of icon labeling issues, but also a solution for solving those issues by a model to predict the label of the image.
For instance, Harrison et al.~\cite{harrison2011kineticons} establish an initial ‘kineticon vocabulary’ containing a set of 39 kinetic behaviors for icon images, such as spin, bounce, running, etc.
Ross et al.~\cite{ross2018examining} identify some common labeling issues in Android apps via analyzing the icon image labeling.
% There are also some works targeting at locating and solving the accessibility issues.
% Zhang et al~\cite{zhang2018robust} leverage the crowd source method to annotate the GUI element without the original content description. They further develop an approach to deploy the interaction proxies for runtime repair and enhancement of  accessibility~\cite{zhang2017interaction} without referring to the source code.
With crowd source method, Zhang et al~\cite{zhang2018robust} annotate GUI elements without content description.
% They also develop a tool to repair runtime and enhance accessibility by deploying the interaction proxies.
% However, these works still need much effort from developers.
However, these works still require support from developers.
Due to the increasingly developed Convolutional Neural Networks (CNNs) technologies, dramatic advances appears in the field of image classification which is applied to automatically annotate tags for images.
Chen et al.~\cite{chen2020lost} analyze the tags associated with the whole GUI artwork collected from Dribbble, and emerge an vocabulary that summarizes the relationship between the tags. 
Based on the vocabulary, they adopt a classification model to recommend the general tags in the GUI, such as "sport", "food", etc.
Different from their work, we predict more fine-grained categories, such as "football", "burger", etc.
And also, they focus on predicting the categories of the whole UI which is subjective to human perception, but the categories of small icons are usually more intuitive.
A similar work to ours is the icon sensitive classification by Xiao et al~\cite{xiao2019iconintent}.
They utilize traditional computer vision techniques like SIFT and FAST to extract the features of icons and classify icons into 8 categories through calculating their similarity.
After the systematically investigation of icons, we discover the fundamental limitations in icons discussed in Section~\ref{empiricalstudy}, in terms of \textit{high cross-class similarity} and \textit{small, transparent and low contrast}. These findings conflict with methods applied in their paper such as applying rotation to augment the dataset. Moreover, we show that deep learning model is fruitful for the icon classification problem than the tradition computer vision technique in Section~\ref{prediction_result}.
In our work, according to the characteristic of icons, we propose a deep learning model to automatically classify icons in a more fine-grained (100) category and also adopt a computer vision technique to detect its primary color.
% The model proposed in our work can automatically recommend the label for icon images and developers can directly use it.
% By supporting these two main features, developers can obtain better code readability during development, thereby increasing the development speed.
% To the best of our knowledge, this is the first work considering developers' requirement and adopting an automated approach to support code readability needs for developers.


\begin{comment}
% Software development organizations want their programmers to maintain to some readable coding called coding guidelines~\cite{meek1983guide,smith1986standards}.
Programmers usually maintain the readability of codes by following coding guidelines designed by software development organizations~\cite{meek1983guide,smith1986standards}.
They usually design their own coding guidelines~\cite{googleguideline,microsoftguideline,appleguideline} depending on what suits their organization best and the types of software they develop.
% Writing descriptions is indispensable for all guidelines, promoting the code readability.
In these code guidelines, description is an indispensable part to ensure the code readability.
% Although it is highly encouraged to follow these guidelines, they are often ignored by developers due to the high-intensity development.
Although code descriptions are highly recommended, they are often ignored by developers due to the high development demand.
% Different from these guidelines, our work predicts the description during the developing process without requiring developers laborious thinking and manual description.
Different from these guidelines, our approach automatically predicts the description for icons without the requirement of time-consuming thinking from developers.
% Technically, we use an image classification model to predict the description of icon image. 
% Image classification problem is the task of assigning an input image one label from a fixed set of categories.
% Deep learning has been applied to image classification widely.
\end{comment}

\begin{comment}
\subsection{Image Classification}
% Convolutional Neural Networks (CNNs) technologies show promise for dramatic advances in the field of image classification. 
Due to the increasingly developed Convolutional Neural Networks (CNNs) technologies, dramatic advances appears in the field of image classification.
There are many research works for improving the performance of the classification model, such as ResNet~\cite{he2016deep}, AlexNet~\cite{krizhevsky2012imagenet}, VGG~\cite{simonyan2014very}, etc.
Most of them investigate the scenes of handwritten digits (MNIST~\cite{lecun1998gradient}), real world images (ImageNet~\cite{deng2009imagenet}, CIFAR-10~\cite{krizhevsky2010convolutional}), flower petals (IRIS~\cite{irisdataset}), news (Fake News~\cite{monti2019fake}), finance (Credit Card Fraud~\cite{dal2014learned}), etc.
A few of them are studying the scene of UI.
For example, Deka et al~\cite{deka2017rico} introduce Rico, a dataset for Android UI screenshots, and further adopt a deep auto-encoder model to detect the layout of text and non-text.
Chen et al~\cite{chen2019gallery} propose an object detection model to decompose 11 types of components from UI screenshots, and present a crowd-sourcing dataset called Gallery D.C.
However, they focus merely on the detection task in UI, such as layout detection and components detection.
In contrast, our goal is to classify the icons to support readability of code.
Chen et al.~\cite{chen2020lost} analyze the tags associated with the whole GUI artwork collected from Dribbble, and emerge an vocabulary that summarizes the relationship between the tags. 
Based on the vocabulary, they adopt a classification model to recommend the general tags in the GUI, such as "sport", "food", etc.
Different from their work, we predict more fine-grained categories, such as "football", "burger", etc.
And also, they focus on predicting the categories of the whole UI which is subjective to human perception, but the categories of small icon designs are usually more intuitive.
% However, they can only predict some general categories such as food, sport, etc.
% because one GUI contains many information, it is hard to predict the fine-grained category, such as burger, football, etc.
% And also, since a GUI contains a large amount of information, the category of GUI biases with the focus of people's attention.
% In addition, since a GUI contains a large amount of components, some GUI are ambiguous. 
% For instance, the type of a GUI with a pair of shoes may be sport rather than shopping.
A similar work to ours is the icon sensitive classification by Xiao et al~\cite{xiao2019iconintent}.
% But their technique is based on traditional computer vision techniques like SIFT and FAST to extract the features of icon and hence classify into 8 categories by calculating their similarity.
They utilize traditional computer vision techniques like SIFT and FAST to extract the features of icon and classify icons into 8 categories through calculating their similarity.
After the systematically investigation of icon designs, we find the fundamental limitations of in icon designs discussed in Section~\ref{empiricalstudy}.
Deep learning model has proven fruitful for the problem than the tradition computer vision technique shown in Section~\ref{prediction_result}, therefore, we propose a deep learning based model to classify icons in a more fine-grained (100) category.
% As we finding the problem of high cross-class similarity in icon designs, deep learning model has proven fruitful for the problem than the tradition computer vision technique.
% Therefore, we propose a deep learning based model to classify icons in a more fine-grained (100) category.
% Since deep learning has shown better performance than the traditional computer vision techniques, we propose a deep learning based model to classify icons in a more fine-grained category.
\end{comment}

==> Auto-Icon+_ An Automated End-to-End Code Generation Tool for Icon Designs in UI Development/semantic.tex <==
\section{Icon Characteristics}
\label{characteristics}
% To address these challenges, we propose an approach for developers that can automatically label unknown icons. 
% Firstly, to reduce the effort of manually designing the classes of icons, we design an label generation method that can automatically decide the classes of icons. 
% Secondly, we utilize the MobileNet V2 model as classifier.
% we collect labels from iconfont website, where user can add labels for each icon when they upload it.
% To reduce the effort of manually designing the classes of icons, we 

% extract the class information from these collected labels and icons via clustering the collected icon labels.
% We convert these labels to word embedding
% There are numerous icon design sharing websites available online. 
% Some of them have rather comprehensive icon library, for example Font Awesome~\cite{?}, Google Material Design Icons~\cite{?}. 

\begin{table}
\caption{The 40 icon classes identified through an iterative open coding of 100k icons from the Iconfont~\cite{iconfont}.}
\centering
\small
\begin{tabular}{p{0.12\textwidth}p{0.45\textwidth}p{0.2\textwidth}c}
    \toprule
    \bf{CLASS} & \bf{ASSOCIATED LABEL} & \bf{EXAMPLES} & \bf{NUMBER} \\
    \midrule
    \bf{\small add} & \small{plus, addition, increase, expand, create} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/15.png}} & 357 \\
    \bf{\small calendar} & \small{date, event, time, planning} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/60.png}} & 324 \\
    \bf{\small camera} & \small{photo, take-photo} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/50.png}} & 355 \\
    \bf{\small chat} & \small{chat-bubble, message, request, comment} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/9.png}} & 372 \\
    \bf{\small complete} & \small{finish, confirm, tick, check, ok, done} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/25.png}} & 432 \\
    \bf{\small computer} & \small{laptop, device, computer-response, desktop} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/17.png}} & 521 \\
    \bf{\small crop} & \small{prune, crop-tool, shear, clipper crop-portrait} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/27.png}} & 436 \\
    \bf{\small download} & \small{file-download, save, import, cloud} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/20.png}} & 444 \\
    \bf{\small edit} & \small{editing, handwriting, pencil, pen, edit-fill, modify} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/56.png}} & 546 \\
    \bf{\small emoji} & \small{amojee, sad, happy, emotion} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/31.png}} & 374 \\
    \bf{\small envelope} & \small{letter, email, mail, inbox} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/43.png}} & 332 \\
    \bf{\small exit} & \small{quit, close, switch-off, logout} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/0.png}} & 404 \\
    \bf{\small flower} & \small{flowers, flower pot, sunflower, valentine-flower} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/44.png}} & 377 \\
    \bf{\small gift} & \small{present, reward, surprise} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/40.png}} & 340 \\
    \bf{\small house} & \small{home, rent, house-area, house asset, building, mall} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/26.png}} & 378 \\
    \bf{\small left} & \small{return, back, prev, backwards} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/16.png}} & 531 \\
    \bf{\small like} & \small{thumb-up, heart, vote, hand-like, upvote, dislike, favourite} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/52.png}} & 386 \\
    \bf{\small location} & \small{gps, direction, compass, navigation} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/11.png}} & 543 \\
    \bf{\small menu} & \small{menu file, card, menufold, menu-line, more, dashboard} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/28.png}} & 351 \\
    \bf{\small minus} & \small{remove, minus (with circle), minus-sign} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/23.png}} & 556 \\
    \bf{\small music} & \small{music-note, music-library, musical-instrument} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/42.png}} & 375 \\
    \bf{\small news} & \small{newspaper, info, announcement} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/18.png}} & 423 \\
    \bf{\small package} & \small{package-up, package-sent, handpackage, personal package} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/39.png}} & 362 \\
    \bf{\small pay} & \small{money, wallet, dollar, commerce} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/32.png}} & 364 \\
    \bf{\small person} & \small{user, avatar, account, customer} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/49.png}} & 562 \\
    \bf{\small photo} & \small{image, picture, camera} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/59.png}} & 481 \\
    \bf{\small play} & \small{playicon, broadcast, play voice, play button, play arrow} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/58.png}} & 498 \\
    \bf{\small question} & \small{ask, faq, information, help, info, support} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/10.png}} & 350 \\
    \bf{\small refresh} & \small{reload, sync, reset, recreate} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/12.png}} & 321 \\
    \bf{\small right} & \small{forward, next, go, arrow-forward} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/24.png}} & 412 \\
    \bf{\small safe} & \small{safe box, safety, safety certificate, lock, secure} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/19.png}} & 476 \\
    \bf{\small search} & \small{investigate, search-engine, magnifier, find, glass} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/5.png}} & 377 \\
    \bf{\small send} & \small{send-arrow, paper-plane, message} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/53.png}} & 318 \\
    \bf{\small settings} & \small{toolbox, gear, preferences, options} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/21.png}} & 317 \\
    \bf{\small shopping} & \small{cart, shopping-bag, checkout} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/30.png}} & 472 \\
    \bf{\small signal} & \small{signal-tower, wave, radio, broadcast} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/55.png}} & 548 \\
    \bf{\small sound} & \small{speaker, sound volume, player} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/36.png}} & 415 \\
    \bf{\small star} & \small{collection, rate, favourite} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/34.png}} & 424 \\
    \bf{\small switch} & \small{switch-on/off, switcher, open, close} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/41.png}} & 319 \\
    \bf{\small text} & \small{word, textbox, font, size} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/54.png}} & 446 \\
    \bf{\small visibility} & \small{visible, show, hide, visibility-off, in-sight} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/37.png}} & 339 \\
    \bf{\small warn} & \small{alarm, warning, error, report, alert} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/35.png}} & 369 \\
    \bf{\small wifi} & \small{wi-fi, wireless, network, signal} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/1.png}} & 429 \\
    \bf{\small zoom-in} & \small{fullscreen, expand, adjust, magnifier} & \parbox[c]{1em}{\includegraphics[width=1in]{icons/3.png}} & 384 \\
    \bottomrule
\end{tabular}
\label{tab:categorization}
\end{table}

In this section, we carry out an empirical study of collaborative icon labelling in online icon design sharing websites to understand its characteristics for motivating the required tool support.
There are numerous online icon design sharing websites such as Font Awesome~\cite{fontawesome}, Google Material Design Icons~\cite{googlematerial}, provide comprehensive icon library to assist designers and developers in designing and coding.
% A main drawback of these websites is that the design is not diverse, that is they formally define an icon matches a label, and vice versa.
In these online icon websites, each label matches only one icon design.
While in real case, one label may have several different designs, revealing the limited diversity of these websites.
In this work, we select Alibaba Iconfont website~\cite{iconfont} as our study subject - not only because it has gained significant popularity among designers' community, but also due to it has became repositories of knowledge with millions of diverse icon designs created by designers.
% Since its foundation in 2014, Alibaba Iconfont has become one of the largest networking platforms for professional designers to share their own icon designs - each comprising human creativity and aesthetics.
To collect icons and associated labels, we built a web crawler based on the Breadth-First search strategy~\cite{najork2001breadth} i.e., collecting a queue of URLs from a seed list, and putting the queue as the seed in the second stage while iterating.
The crawling process continued from December 12, 2019 to July 1, 2020 with a collection of 100k graphical icons.
% Note that these graphical designs are diverse including icon, logo, illustration, clip art, branding, etc.

\subsection{Overview}
\label{empiricalstudy}
% Within the Alibaba Iconfont site, the design creators can add their personal subjective label for their design work.
% To provide readers with a better understanding of detailed semantic embedded in the icon design, we adopt the association rule mining~\cite{?} and community detection~\cite{?} for visualizing the collected icon labels.

During the process of open coding the categories of icons semantic, we find that one label can be written in different styles. 
For example, the label "crop" can be written in not only its standard format, but also its derivations synonyms like "prune", "clip", "crop-tool".
Moreover, due to the icon labelling process in Iconfont is informal and icon designs are contributed by thousands of designers with very diverse technical and linguistic backgrounds the same concept may labeled in many user defined terms such as "crop-fill", "crop-portrait", "icon-crop-solid-24px".
The wide presence of forms poses a serious challenge to icon classification task.
For example, the icon can be described to the class of "crop" or "clip", which makes sense in both classes.

To address the problem, we adopted association rule mining~\cite{agrawal1994fast} to discover label correlations from label co-occurrences in icons.
We leveraged the visual information from the icons and textual information from the labels to group a pair-wise correlation of labels.
For measuring the visual similarity, we adopted the image similarity score MSE~\cite{wang2004image} $sim_{vis(x,y)}$ to calculate the likelihood if two icons are the same.
For measuring the textual information, we first trained a word embedding~\cite{mikolov2013distributed} model to convert each label into a vector that encodes its semantic.
Then we defined a lexical similarity threshold based on the string edit distance~\cite{levenshtein1966binary} $sim_{text(x,y)}$ to check if two labels are similar enough in the form.
The labels are grouped as a pair-wise correlation if $sim_{vis(x,y)}\geq0.9$ or $sim_{text(x,y)}\geq0.9$.
As we wanted to discover the semantics and construct a lexicon of categories, we found frequent pairs of labels.
A pair of labels is frequent if the percentage of how many icons are labelled with this pair of tags compared with all the icons are above the minimum support threshold $t_{sup}\geq0.001$.
Given a frequent pair of labels $\{t_1, t_2\}$, association rule mining generated an association rule $t_1 \Rightarrow t_2$ if the confidence of the rule $t_{conf}\geq0.2$.
Given the mined association rules, we constructed an undirected graph $G(V, E)$, where the node set $V$ contains the labels appearing in the association rules, and the edge set $E$ contains undirected edges $<t_1, t_2>$ (i.e., pair of label associations) if the two labels have the association $t_1 \Rightarrow t_2$ or $t_2 \Rightarrow t_1$.
Note that the graph is undirected because association rules indicate only the correlations between antecedent and consequent.
% Each edge has a confidence attribute indicating the strength of the technology association.
All threshold values were carefully selected through manually check, considering the balance between the information coverage and overload.

To identify the set of frequently occurred icon label categories, we performed an iterative open coding of most frequent co-occurring labels (or approximately 9.2\% of the dataset 542,334 in total) with existing expert lexicon of categories in books and websites such as \textit{Google’s Material icon set}~\cite{googlematerial}, \textit{IBM's Design Language of Iconography}~\cite{ibmicon} and \textit{Design Pattern Gallery}~\cite{neil2014mobile}.
Two researchers from our team independently coded the categories of these labels, noting any part of the initial vocabulary.
Note that both researchers have design experiences in both icons and UI development.
After the initial coding, the researchers met and discussed the discrepancies and the set of new label categories until consensus was reached.
% Researchers assigned labels using an input field that autocompleted on categories already in the lexicon (including ‘not an icon’), and created new categories when necessary.
% As part of this process, we identified distinguishing features for visually-similar icons to remove ambiguity. For example, we require that icons have a vertical line after the arrows to distinguish them from the visually-similar class
% We yield \sidong{100} main semantic icon categories as seen in Figure~\ref{?}.
A semantic icon categories can be seen in Table~\ref{tab:categorization}.
We observed two distinct characteristics in icons compared to the physical-world objects.

\textbf{High cross-class similarity:} 
Icons of different classes often have similar size, shape and visual features.
The visual differences to distinguish different classes of icons can be subtle, particularly small widgets are differentiated by small visual cues.
For example, the difference between "newspaper" and “file" lies in a text of news at the top/bottom side of "newspaper", while a plus/minus symbol distinguishes
"zoom\underline{ }in"/"zoom\underline{ }out" from "search".
In addition, direction is also an important aspect to distinguish classes. For example, the inclined waves represent "signal" and the upward waves represent "wifi".
Existing object classification tasks usually deal with physical objects with distinct features across classes, for example, fishes, flowers, hockey and people in the popular ImageNet dataset~\cite{deng2009imagenet}.
High cross-class similarity affects classification as the class can be not easily distinguished.

\textbf{Small, transparent and low contrast:} 
To make UI unique and stylish in the screen, icons are usually small and partially transparent, such as the last icon in the "minus" class shown in Table~\ref{tab:categorization}.
The transparent icons in the UIs do not cause vision conflict, while they are less visible when separated from the background context.
For example, the first icon in the "text" class in Table~\ref{tab:categorization} is an icon with low color contrast and uses transparency and shadow to stress contrast.
While the contrast of the object is obvious in the current dataset, especially apparent in the greyscale format such as MNIST dataset~\cite{lecun1998gradient}.
% Transparent and low contrast decrease the ability for model to extract feature of images~\cite{xu2015salient,mu2018salient}.
% And small icon classification suffers from vanishing gradient problem as it may disappear somewhere in the middle of the model~\cite{hochreiter1998vanishing,vanish}.


\noindent\fbox{
    \parbox{0.98\textwidth}{
        Existing icon sharing sites contain a wide presence of forms of labeling.
        Based on different background knowledge, designers use different same-meaning labels to annotate the same icon.
        Such limitation not only confirms our finding of difficulty of commenting in Section~\ref{rq2}, but also hinders the potential challenge in classification task.
        % Therefore, a data mining approach captured visual and textual information is applied to construct a lexicon in icons.
        Therefore, a data mining approach capturing visual and textual information is applied to construct a lexicon in icons.
        % By observing the lexicon, we find that two distinct characteristics of icon which pose challenges for the icon classification task. 
        By observing the lexicon, we find that two distinct characteristics of icon different from the existing physical object orientated dataset.
    }
}
